BOP-Elites, a Bayesian Optimisation Approach to Quality Diversity Search with Black-Box descriptor functions

Quality Diversity (QD) algorithms such as MAP-Elites are a class of optimisation techniques that attempt to find many high performing points that all behave differently according to a user-defined behavioural metric. In this paper we propose the Bayesian Optimisation of Elites (BOP-Elites) algorithm. Designed for problems with expensive black-box fitness and behaviour functions, it is able to return a QD solution-set with excellent final performance already after a relatively small number of samples. BOP-Elites models both fitness and behavioural descriptors with Gaussian Process (GP) surrogate models and uses Bayesian Optimisation (BO) strategies for choosing points to evaluate in order to solve the quality-diversity problem. In addition, BOP-Elites produces high quality surrogate models which can be used after convergence to predict solutions with any behaviour in a continuous range. An empirical comparison shows that BOP-Elites significantly outperforms other state-of-the-art algorithms without the need for problem-specific parameter tuning.

==> surrogate_me.tex <==
% Applications
SAIL has been primarily applied as a tool for exploration in search spaces where simulations or experiments are very expensive, such as aerodynamic design and materials science~\citep{sail_ecj, sail_aiaa, sail_gecco, produqd, sphen, sen2021integration}.

% Extensions
The general framework introduced by SAIL for adapting Bayesian optimization to QD has been adapted to predict descriptors along with objectives~\citep{sphen} in order to find solutions with specific features; to apply EI rather than UCB in order to chose the single best sample to evaluate in the most expensive use cases~\citep{bop_elites}, and as a component in a larger generative design process that is iteratively applied to narrow in on promising design spaces~\citep{produqd}.

% Non-GP
Surrogate-assisted approaches outside of Bayesian optimization, which seek only to generate a high performing archive rather than an active model, have shown promise in accelerating problems which are both high-dimensional and expensive~\citep{dsame_gecco, dsame_iclr}.

